Rational Recurrences

Despite the tremendous empirical success of neural models in natural language processing, many of them lack the strong intuitions that accompany classical machine learning approaches. Recently, connections have been shown between convolutional neural networks (CNNs) and weighted finite state automata (WFSAs), leading to new interpretations and insights. In this work, we show that some recurrent neural networks also share this connection to WFSAs. We characterize this connection formally, defining rational recurrences to be recurrent hidden state update functions that can be written as the Forward calculation of a finite set of WFSAs. We show that several recent neural models use rational recurrences. Our analysis provides a fresh view of these models and facilitates devising new neural architectures that draw inspiration from WFSAs. We present one such model, which performs better than two recent baselines on language modeling and text classification. Our results demonstrate that transferring intuitions from classical models like WFSAs can be an effective approach to designing and understanding neural models.

==> fig/fsa-tikzstyle.tex <==
\tikzset{
  ->,
  >=stealth', % makes the arrow heads bold
  inner frame sep=-2mm,
  node distance=3cm,
  auto,
  every state/.style={
    thick,
  },
  every node/.style={
    above=0cm,
  },
  initial text=$ $, % sets the text that appears on the start arrow
}


==> text/notes.tex <==
\section{Notes for Camera Ready}
\subsection{Breaking Semiring Laws}
IndRNN is proposed in \citet{li2018indrnn}, where the affine transformation along the recurrent direction is constrained to be diagonal. More precisely:
\begin{align}
\label{eq:indrnn}
\mathbf{c}_t = \tanh\left(\mathbf{w}\odot\mathbf{c}_{t-1} + \mathbf{b}\right),
\end{align}
where $\mathbf{w}$ and $\mathbf{b}$ are part of the learned parameters.
Comparing it to Example~\ref{example:simple}, it is easy to verify that
Equation~\ref{eq:indrnn} would have been rational, if not for the $\tanh$.

I know from a personal communication with Tao Lei that the most recent version of SRU (submitted to EMNLP) uses this recurrent updates. Therefore it might be an interesting discussion to include into the revised version.

\subsection{Composition of Rational RNNs}
The idea is to two rational RNNs, one to compute the hidden states, and the other used to compute the forget gate. 
More precisely:
\begin{subequations}
	\begin{align}
	\mathbf{f}^{(j)}_t&=\bm{\sigma}\bigl(\mathbf{W}^{(j)}_{f}\mathbf{v}_{t} + \mathbf{b}^{(j)}_{f}\bigr), \quad j=1,2\\
	\mathbf{u}^{(j)}_t&=(1-\mathbf{f}^{(j)}_t) \odot\mathbf{W}^{(j)}_{u} \mathbf{v}_{t},\quad j=1,2\\
	\mathbf{c}^{(j)}_t &= \mathbf{c}^{(j)}_{t-1}\odot\mathbf{f}_t^{(j)} + \mathbf{u}_t^{(j)},\quad j=1,2 \\
	\mathbf{c}_t &= \bm{\sigma}(\mathbf{c}^{(1)}_{t})\odot\mathbf{c}_{t-1}
	+ \left(\mathbf{1} - \bm{\sigma}(\mathbf{c}^{(1)}_{t}) \right)\odot\mathbf{c}^{(2)}_{t}\label{eq:rec}
	\end{align}
\end{subequations}
$\mathbf{c}^{(j)}_t$ shall be two (unigram) rational RNNs, just as what we have already done;
the interesting part is that $\mathbf{c}^{(1)}_t$ is used as the forget gate,
while $\mathbf{c}^{(2)}_t$ as content cell when computing
hidden states $\mathbf{c}_t$, which will be used for onward computation.

In this way, both the content cell and the forget gate would depend on the entire history, in addtion to the current input token. 
In this sense, this model might perform better in practice.

My questions:
\begin{itemize}
	\item I guess the resulting model is not a WFSA anymore. Does this correspond to any classical techniques in the WFSA literature?
	\item Does this model appear interesting to you? Do you think it makes sense to include this into the camera-ready?
\end{itemize}
